Federated Koopman-Reservoir Learning for Large-Scale Multivariate Time-Series Anomaly Detection

The proliferation of edge devices has dramatically increased the generation of multivariate time-series (MVTS) data, essential for applications from healthcare to smart cities. Such data streams, however, are vulnerable to anomalies that signal crucial problems like system failures or security incidents. Traditional MVTS anomaly detection methods, encompassing statistical and centralized machine learning approaches, struggle with the heterogeneity, variability, and privacy concerns of large-scale, distributed environments. In response, we introduce FedKO, a novel unsupervised Federated Learning framework that leverages the linear predictive capabilities of Koopman operator theory along with the dynamic adaptability of Reservoir Computing. This enables effective spatiotemporal processing and privacy preservation for MVTS data. FedKO is formulated as a bi-level optimization problem, utilizing a specific federated algorithm to explore a shared Reservoir-Koopman model across diverse datasets. Such a model is then deployable on edge devices for efficient detection of anomalies in local MVTS streams. Experimental results across various datasets showcase FedKO's superior performance against state-of-the-art methods in MVTS anomaly detection. Moreover, FedKO reduces up to 8x communication size and 2x memory usage, making it highly suitable for large-scale systems.

==> SDMSections_Full/abstract.tex <==
\begin{abstract}
The advent of IoT has significantly boosted data generation, particularly in multivariate time-series (MVTS) which are vital for real-world applications ranging from industrial monitoring to smart city management. However, these data streams are prone to be disrupted by anomalous activities, signaling critical issues like system malfunctions or security breaches. 
Conventional MVTS anomaly detection methods, encompassing statistical and centralized machine learning approaches, struggle with the heterogeneity, variability, and privacy challenges of IoT environments. 
In this study, we introduce \textsc{FedKO}, a novel Federated Learning framework that leverages the linear predictive capabilities of Koopman operator theory along with the dynamic adaptability of Reservoir Computing. This enables effective spatiotemporal processing and privacy-preserving anomaly detection in MVTS IoT environments. 
\textsc{FedKO} is formulated as a bi-level optimization problem, utilizing a tailored federated algorithm to explore a shared Koopman-Reservoir model across diverse datasets. Such a model is then deployable on individual devices for efficient detection of anomalies in local MVTS streams. Experimental results across various datasets showcase \textsc{FedKO}'s superior performance against state-of-the-art methods in MVTS anomaly detection. Moreover, \textsc{FedKO} reduces up to 8$\times$ communication size and 2$\times$ memory usage, making it highly suitable for IoT.
\end{abstract}

\begin{IEEEkeywords}
	Federated Learning, Koopman Operator, Reservoir Computing, Multivariate Time-Series, IoT, Anomaly Detection
\end{IEEEkeywords}

% in linear dynamical system modeling
%not only enhance performance but also reduces training and computational complexity in MVTS analysis, enabling scalability and real-time analysis capabilities, crucial in resource-constrained IoT environments. 
%create an efficient, privacy-preserving MVTS anomaly detection framework. 

==> SDMSections_Full/analysis.tex <==
\subsection{Computational Analysis}

==> SDMSections_Full/biography.tex <==
\section{Biography Section}

%\vspace{11pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/tunganh.jpg}}]{Tung-Anh Nguyen} received his B.E. degree in Electronics and Telecommunications from Hanoi University of Science and Technology (HUST), Vietnam, in 2016. He received his MSC degree in Computer and Information Science from Korea University, Korea, in 2019. Currently, he is pursuing a PhD degree in Computer Science at DUAL group, Faculty of Engineering, the University of Sydney (USyd), NSW, Australia. His research interests include Distributed Machine Learning, Federated Learning, Blockchain and Optimization for Distributed Systems.
\end{IEEEbiography}
%\vspace{11pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/long.jpg}}]{Long Tan Le} received B.E. degree with honours in Computer Engineering from Ho Chi Minh City University of Technology (HCMUT) in 2018. He was a researcher at the Faculty of Computer Science and Engineering, HCMUT from 2018 to 2021. Currently, he is pursuing a Ph.D degree in Computer Science at the Faculty of Engineering, the University of Sydney (USyd). His research interests include Machine Learning, Federated Learning, and their applications for next-generation networking.
\end{IEEEbiography}
%\vspace{11pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/josh.jpeg}}]{Tuan Dung Nguyen} received his B.S. in computer science from the University of Melbourne and is currently an M.Phil. student at the Australian National University, where he is a part of the Computational Media Lab. His research interests span machine learning, convex optimization, distributed computing and social network analysis.

\end{IEEEbiography}
%\vspace{11pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/wei_bao.jpg}}]{Wei Bao} (Member, IEEE) received the BE degree in communications engineering from the Beijing University of Posts and Telecommunications, Beijing, China, in 2009, the MASc degree in electrical and computer engineering from the University of British Columbia, Vancouver, Canada, in 2011, and the PhD degree in electrical and computer engineering from the University of Toronto, Toronto, Canada, in 2016. He is currently a senior lecturer with the School of Computer Science, University of Sydney, Sydney, Australia. His research covers the area of network science, with particular emphasis on Internet of things, mobile computing, edge computing, and distributed learning. He received the Best Paper Awards in ACM International Conference on Modeling, Analysis and Simulation of Wireless and Mobile Systems (MSWiM) in 2013 and 2019 and IEEE International Symposium on Network Computing and Applications (NCA) in 2016.
\end{IEEEbiography}
%\vspace{11pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/suranga.jpeg}}]{Suranga Seneviratne} (Senior Member, IEEE) received the bachelor’s degree from University of Moratuwa, Sri Lanka, in 2005, and the Ph.D. degree from University of New South Wales, Australia, in 2015. He is a Lecturer of Security with the School of Computer Science, The University of Sydney. His current research interests include privacy and security in mobile systems, AI applications in security, and behavior biometrics. Before moving into research, he worked nearly six years in the telecommunications industry in core network planning and operations
\end{IEEEbiography}
%\vspace{11pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/choong_seong_hong.jpg}}]{Choong Seon Hong} (S’95-M’97-SM’11) received the B.S. and M.S. degrees in electronic engineering from Kyung Hee University, Seoul, South Korea, in 1983 and 1985, respectively, and the Ph.D. degree from Keio University, Tokyo, Japan, in 1997. In 1988, he joined KT, Gyeonggi-do, South Korea, where he was involved in broadband networks as a member of the Technical Staff. Since 1993, he has been with Keio University. He was with the Telecommunications Network Laboratory, KT, as a Senior Member of Technical Staff and as the Director of the Networking Research Team until 1999. Since 1999, he has been a Professor with the Department of Computer Science and Engineering, Kyung Hee University. His research interests include future Internet, intelligent edge computing, network management, and network security. Dr. Hong is a member of ACM, IEICE, IPSJ, KIISE, KICS, KIPS, and OSIA. He was an Associate Editor of the IEEE TNSM and the IEEE JSAC.
\end{IEEEbiography}
%\vspace{11pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/nguyen.jpg}}]{Nguyen H. Tran} (S’10-M’11-SM’18) received BS and PhD degrees (with best PhD thesis award), from HCMC University of Technology and Kyung Hee University, in electrical and computer engineering, in 2005 and 2011, respectively. Dr Tran is an Associate Professor at the School of Computer Science, The University of Sydney. He was an Assistant Professor with Department of Computer Science and Engineering, Kyung Hee University, from 2012 to 2017. His research group has special interests in Distributed compUting, optimizAtion, and machine Learning (DUAL group). He received several best paper awards, including IEEE ICC 2016 and ACM MSWiM 2019. He receives the Korea NRF Funding for Basic Science and Research 2016-2023, ARC Discovery Project 2020-2023, and SOAR award 2022-2023. He has been on the Editorial board of several journals such as IEEE Transactions on Green Communications and Networking (2016-2020), IEEE Journal of Selected Areas in Communications 2020, and IEEE Transactions on Machine Learning in Communications Networking (2022-).
\end{IEEEbiography}
%\vspace{11pt}
\vfill

==> SDMSections_Full/convergence.tex <==
\section{\textsc{FedPCA}: Convergence Analysis}
\label{sec:convergence_analysis}
In this section, we present a theoretical analysis to understand the convergence properties of \textsc{FedPG} and \textsc{FedPE} within FedPCA framework. To begin with, we consider a FL environment with $N$ clients, indexed by $i=1,2,\ldots, N$, and introduce the following notations for the analyses:
%Let $i=1,2, \ldots, N$ be the indice of $i$-th client.
\begin{enumerate}
    \item $\mathcal{S}^k \subset \{1,2, \ldots, N\}$: denotes the subset of clients selected in the $k$-th iteration.
    \item $k(i)$: denotes the latest iteration at which the client $i$ has its model updated.
\end{enumerate}

%The following convergence analysis is conducted for both FedPG and FedPE. 
The orthonormality constraint in \eqref{Prob:pca_decentralized_admm} is a critical component for our proposed method. While \textsc{FedPE} handles this by introducing a surrogate linear constraint in (\ref{eqn:Hi}), \textsc{FedPG} relaxes this by leveraging projected gradient descent on Grassmann manifolds. Hence, to ensure the generality of our framework, we employ the augmented Lagrangian \eqref{eqn: lagrange} and rewrite it to adapt for the convergence analysis of both algorithms as follows.
\begin{equation}
    \label{eqn: aug_lagrangian}
    \begin{split}
	\mathcal{L}(\{U_i\}, Z, \{Y_i\}) &= \SumLim{i=1}{N} f_i(U_i) + \SumLim{i=1}{N} Y_i^\top (U_i - Z) \\
     & \qquad\qquad\qquad + \frac{\rho_i}{2} \SumLim{i=1}{N} \norm{U_i - Z}^2_F \\
     \mathrm{s.t.} \quad  U_i^\top U_i & = I.
    \end{split}
\end{equation}

In addition, we modify the global update \eqref{ADMM_PCA_update_Z} at $CO$ by following:
\begin{equation}
    \label{eqn:Z_update}
    Z^{k+1} = \frac{1}{|S_k|} \sum_{i \in S_k}^{} U_i^{k}
\end{equation}

Accordingly, the local updates for $U_i^{k+1}$ in~\eqref{ADMM_PCA_update_U_i} and $Y_i^{k+1}$ in~\eqref{ADMM_PCA_update_Y_i} at a selected client $i$ will be changed as listed below.
%Step 1:

\begin{align}
    U_i^{k+1} & = \underset{U_i}{\operatorname{\argmin}}  \BigC{f_i(U_i) + \innProd{Y_i^k, U_i - Z^k}_F \nonumber \\
    & \qquad\qquad\qquad\qquad+ \frac{\rho_i}{2} \SumLim{i=1}{N} \norm{U_i - Z}^2_F} \label{eqn:Ui_update} \\
     & \mathrm{s.t.} \quad  U_i^\top U_i = I \nonumber \\      
     Y_i^{k+1} & = Y_i^k + \rho \BigP{U_i^{k+1} - Z^{k+1}} \label{eqn:Yi_update}
\end{align}
%Step 2:

It is worth noting that this modification does not affect the performance of \textsc{FedPE} and \textsc{FedPG} since the update results will be the same after one iteration.


\vspace{5pt}
\textbf{Assumption.}
We first make the following assumptions:
\begin{itemize}
	\item A1: For each client's objective function $f_i, \forall i = 1, \ldots, N$ there exists a constant $L_i \geq 0$ such that for any two points $U_i, Z_i$, the gradient of $f_i$ satisfies the Lipschitz condition:  $$\left\|\nabla f_i\left(U_i\right)-\nabla {f_i}\left(Z_i\right)\right\|_F \leq L_i\left\|U_i-Z_i\right\|_F, \forall i$$
	
	\item A2: For all $i$, the penalty parameter $\rho_i$ is chosen large enough such that the $U_i$ sub-problem (\ref{eqn:Ui_update}) is strongly convex with modulus $\mu_i\left(\rho_i\right)$.

    \item A3: $\gL(x)$ is bounded from below, i.e.,
        $$\underline{\gL} \defeq \min_{X} \gL(X) > - \infty$$
\end{itemize}

\begin{remark}
Assumption A1 and A3 are standard in analyzing convergence properties for ADMM. Under Assumption A2, as $\rho_i$ increases, the subproblem \eqref{eqn:Ui_update} will be eventually strongly convex with respect to $U_i$. The associated strong convexity modulus $\mu_i\left(\rho_i\right)$ is a
monotonic increasing function of $\rho_i$.  
\end{remark}
%To establish a convergence guarantee  ADMM, we aim to show the following... 

To establish a convergence guarantee of \textsc{FedPE} and \textsc{FedPG}, we aim to show the following. Start with the variables $(\{ U_i^k \}, Z^k, \{ Y_i^k \})$. After $T$ rounds (i.e., after all clients have participated at least once since iteration $k$), the new variables $(\{ U_i^{k+T} \}, Z^{k+T}, \{ Y_i^{k+T} \})$ lead to decrease in the global augmented Lagrangian $\gL$. Then we show these variables will converge to a local stationary point of $\gL$. Notably, our analysis employs matrix variables, in constrast to other ADMM-based methods using vector variables~\cite{giesen2016distributed, Hong2015,Chang2016, admm_nonconvex}
%\blue{Our problem relies on matrix variables, unlike other ADMM-based algorithms using vector variables~\cite{giesen2016distributed, Hong2015,Chang2016, admm_nonconvex}}
%\vspace{-7pt}
\subsection{Bound on the Successive Difference of Dual Variables}

We establish an upper bound for the successive difference of the dual variables $Y_i$ in terms of the primal variables $U_i$.

\begin{lemma}
    Suppose Assumptions A1 hold, then we have
    \begin{equation}
    \label{eqn:lemma1}
        \left\|Y_i^{k+1}-Y_i^k\right\|_F^2 \leq L_i^2\left\|U_i^{k+1}-U_i^k\right\|_F^2, \forall i, \forall k
    \end{equation}
    \label{lemma:diff_dual}
\end{lemma}

\begin{proof}
In the case of $i \not\in S^k$, (\ref{eqn:lemma1}) is true because both sides of (\ref{eqn:lemma1}) are equal to zero. When $i \in S^k$, we have below equation from optimal condition for (\ref{eqn:Ui_update}).
\begin{equation}
    \label{eqn:lemma1-1}
    \nabla {f_i}\left(U_i^{k+1}\right) + Y_i^{k+1} + \rho_i(U_i^{k+1} - Z^{k+1}) = 0
\end{equation}

Substituting (\ref{eqn:lemma1-1}) to the dual variable update (\ref{eqn:Yi_update}), the following equation is derived.
\begin{equation}
    \label{eqn:*}
    \nabla {f_i}\left(U_i^{k+1}\right) = -Y_i^{k+1}
\end{equation}

Combining with Assumption $A1$, and noting that for any given $i$, $U_i$ and $Y_i$ are updated in the same iteration, we obtain for all $i \in {S^k} / \{0\}$ :
\begin{equation*}
\begin{split}
\left\|Y_i^{k+1}-Y_i^k\right\|_F &  = \left\|\nabla {f_i}\left(U_i^{k+1}\right)-\nabla {f_i}\left(U_i^{k(i)}\right)\right\|_F \\
&= \left\|\nabla {f_i}\left(U_i^{k+1}\right)-\nabla {f_i}\left(U_i^{k(i)}\right)\right\|_F \\
&\leq L_i\left\|U_i^{k+1}-U_i^{k(i)}\right\|_F = L_i\left\|U_i^{k+1}-U_i^k\right\|_F
\end{split}
\end{equation*}
\end{proof}

\subsection{Bound for the Augmented Lagrangian}
Next, we show that the augmented Lagrangian \eqref{eqn: aug_lagrangian} can be decreased sufficiently and bounded below.

\begin{lemma}%[Decrease in the augmented Lagrangian]
Suppose Assumption A1, A2 and A3 hold, then the augmented Lagrangian is bounded as follows.
\begin{equation*}
\begin{split}
	& \mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1},\left\{Y_i^{k+1}\right\}\right)-\mathcal{L}\left(\left\{U_i^k\right\}, Z^k,\left\{Y_i^k\right\}\right) \\
	\leq & \sum_{i \in S^{k}}\left(\frac{L_i^2}{\rho_i}-\frac{\rho_i}{2}\right)\left\|U_i^{k+1}-U_i^k\right\|_F^2-\frac{\mu_i}{2}\left\|Z^{k+1}-Z^k\right\|^2
\end{split}
\end{equation*}
\label{lemma:auglag_decrease}
\end{lemma}
\begin{proof}
For each client $i \in S^k$, we can split the successive difference of the augmented Lagrangian by following.
\begin{equation}
\begin{split}
	& \mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1},\left\{Y_i^{k+1}\right\}\right)-\mathcal{L}\left(\left\{U_i^k\right\}, Z^k,\left\{Y_i^k\right\}\right) \\
	& = \underbrace{\mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1},\left\{Y_i^{k+1}\right\}\right)-\mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1},\left\{Y_i^k\right\}\right)}_A \\
	& +\underbrace{\mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1},\left\{Y_i^k\right\}\right)-\mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^k,\left\{Y_i^k\right\}\right)}_B \\
	& +\underbrace{\mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^k,\left\{Y_i^k\right\}\right)-\mathcal{L}\left(\left\{U_i^k\right\}, Z^k,\left\{Y_i^k\right\}\right)}_C
\end{split}
\label{eq:augLag:split}
\end{equation}

\textbf{Bounding Term A.} The first term in \eqref{eq:augLag:split} can be bounded as follows.
\begin{equation}
\begin{split}
	& \mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1},\left\{Y_i^{k+1}\right\}\right)-\mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1},\left\{Y_i^k\right\}\right) \\
	& =\sum_{i=1}^N\left\langle Y_i^{k+1}-Y_i^k, U_i^{k+1}-Z^{k+1}\right\rangle_F \\
	& \stackrel{(a)}{=} \sum_{i \in S^{k}} \frac{1}{\rho_i}\left\|Y_i^{k+1}-Y_i^k\right\|_F^2 
\end{split}
\label{eq:termA}
\end{equation}
where (a) is achieved by using (\ref{eqn:Yi_update}).

\textbf{Bounding Term B.} The second term in \eqref{eq:augLag:split} can be bounded as follows.
\begin{equation}
\begin{split}
	& \mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1}, Y^k\right)-\mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^k,\left\{Y_i^k\right\}\right) \\
	& \stackrel{(A2)}{\leq} \sum_{i=1}^N \Big(\left\langle\nabla_{U_i} \mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1}, Y^k\right), U_i^{k+1}-U_i^k\right\rangle \\
    & \hskip14em\relax -\frac{\mu_i}{2}\left\|U_i^{k+1}-U_i^k\right\|_F^2 \Big) \\
	& \stackrel{(b)}{=} -\sum_{i \in S^{+}} \frac{\mu_i}{2}\left\|U_i^{k+1}-U_i^k\right\|_F^2 .
\end{split}
\label{eq:termB}
\end{equation}
where (b) is trivially true in the case of $i \not\in S^k$ as $U_i^{k+1}=U_i^k$. In the case of $i \in S^k$, the $\nabla_{U_i} \mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1}, \{Y_i^k\}\right)=0$ because of optimal condition of (\ref{eqn:Ui_update}).

\textbf{Bounding Term C.} The third term in \eqref{eq:augLag:split} can be bounded as follows.
\begin{equation}
\begin{split}
	& \mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^k, \{Y_i^k\}\right)-\mathcal{L}\left(\left\{U_i^k\right\}, Z^k, \{Y_i^k\}\right) \\
	& \stackrel{(c)}{\leq} \sum_{i=1}^N \Big(\left\langle \nabla_{Z} \mathcal{L}\left(\left\{U_i^k\right\}, Z^{k+1}, \{Y_i^k\}\right), Z^{k+1}-Z^k\right\rangle \\
    & \hskip14em\relax-\frac{\gamma}{2}\left\|Z^{k+1}-Z^k\right\|_F^2\Big) \\
	& \stackrel{(d)}{=} \sum_{i \in S^{k}}-\frac{\gamma}{2}\left\|Z^{k+1}-Z^k\right\|_F^2 .
\end{split}
\label{eq:termC}
\end{equation}
where in (c) we used the fact that $\mathcal{L}\left[\left\{U_i\right\}, Z, \{Y_i\}\right\}$ is strongly convex w.r.t. $Z$. 

For (d), it is trivially true if $i \not \in S^k$ as $U_i^{k+1}=U_i^k$. When $i\in S^k$, the $\nabla_Z \mathcal{L}\left(\left\{U_i^k\right\}, Z^{k+1}, \{Y_i^k\}\right)=0$ because of the optimal condition of (\ref{eqn:Ui_update}).

\textbf{Sufficient decease.} Combining the inequalities \Cref{eq:termA}, \Cref{eq:termB} and \Cref{eq:termC} together, we have 
\begin{equation}
\begin{split}
    & {A+B+C} \\ 
    & = \mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1},\left\{Y_i^{k+1}\right\}\right)-\mathcal{L}\left(\left\{U_i^k\right\}, Z^k,\left\{Y_i^k\right\}\right) \\ & \leq \sum_{i \in S^k}-\frac{\gamma}{2}\left\|Z^{k+1}-Z^k\right\|_F^2
      +\left(\frac{L_i^2}{\rho_i}-\frac{\mu_i}{2}\right)\left\|U_i^{k+1}-U_i^k\right\|_F^2 
\end{split}
\label{eq:suff_dec}
\end{equation}
%\hskip10em\relax
This implies that the value of the augmented Lagrangian will always decrease if the following condition is satisfied:
\begin{equation}
    \rho_i \mu_i \geq 2 L_i^2
    \label{eq:condition}
\end{equation}

\textbf{Lower bound for the augmented Lagragian.} We continue showing that $\mathcal{L}\left(\left\{U_i^{k}\right\}, Z^{k}, \{Y_i^{k}\}\right)$ convergence, i.e., $\mathcal{L}$ is bounded below. 
\begin{equation*}
\begin{split}
	& \mathcal{L}\left(\left\{U_i^{k+1}\right\}, Z^{k+1}, \{Y_i^{k+1}\}\right) \\
    & =  \sum_{i=1}^N\Big(f_i\left(U_i^{k+1}\right) +\left\langle Y_i^{k+1}, U_i^{k+1}-Z^{k+1}\right\rangle \\
    &  \hskip14em\relax + \frac{\rho_i}{2}\left\|U_i^{k+1}-Z^{k+1}\right\|_F^2\Big)\\
    & \stackrel{(e)}{=}\sum_{i=1}^N\Big(f_i\left(U_i^{k+1}\right) +\left\langle\nabla f\left(U_i^{k+1}\right), Z^{k+1}-U_i^{k+1}\right\rangle \\
    & \hskip14em\relax +\frac{\rho_i}{2}\left\|U_i^{k+1}-Z^{k+1}\right\|_F^2\Big) \\
    & \stackrel{(f)}{\geq} \sum_{i=1}^N f_i\left(Z^{k+1}\right)=\underline{\gL}\left(Z^{k+1}\right)
\end{split}
\end{equation*}
where (e) can be explained as following:

(e.1) If $i \in S^{k}$, based on (\ref{eqn:*}):
\[\left\langle Y_i^{k+1}, U^{k+1}-Z^{k+1}\right\rangle=\left\langle\nabla_f\left(U_i^{k+1}\right), Z^{k+1}-U^{k+1}\right\rangle\]

(e.2) If $i \notin S^{k}$, $Y_i^{k+1}=Y_i^k=Y_i^{k(i)}$, $U_i^{k+1}=U_i^k=U^{k(i)}$
\begin{equation*}
    \begin{split}
	&\left\langle Y_i^{k+1}, U_i^{k+1}-Z^{k+1}\right\rangle \\
    & =\left\langle\nabla f\left(U_i^{k(i)}\right), Z^{k+1}-U_i^{k(i)}\right\rangle \\
	&=\left\langle\nabla f\left(U_i^{k+1}\right), Z^{k+1}-U_i^{k+1}\right\rangle
\end{split}
\end{equation*}

From combining (e.1) and (e.2), we deduce that (e) holds true. Consequently, due to the Lipschitz continuity of the gradient of $f_i$, (f) is also true.
\end{proof}

\begin{remark}
    \Cref{lemma:auglag_decrease} shows that the augmented Lagrangian decreases by a sufficient amount after each iteration. In practice, however, the penalty parameter  $\rho$ is difficult to estimate. Hence, for our experiments, we fine-tune $\rho$ from a predefined range of values to select the best one.
\end{remark}

\subsection{Convergence of the augmented Lagrangian}
\label{ap:thrm_proof:auglag_convergence}
Here, we combine Lemma \eqref{lemma:diff_dual} and \eqref{lemma:auglag_decrease} to establish the following theorem.

\begin{theorem}
    Suppose the following are true:
    \begin{itemize}
        \item After $T$ iterations, all clients have participated in training at least once.
        \item The global loss function $\mathcal{L}(Z^{k}, \{ U_i^{k} \}, \{ Y_i^{k} \})$ is bounded below by a finite quantity $\underline{\gL}$.
        \item The hyperparameter $\rho_i$ for the augmented Lagrangian is chosen such that $\rho_i \mu_i \geq 2 L_i^2$.
    \end{itemize}
    Then the augmented Lagrangian $\gL$ will monotonically decrease and is convergent to a quantity of at least $\underline{\gL}$. Further, for all $i=1, \dots, N$ we have $\lim_{k \rightarrow \infty} \norm{Z^{k+T} - U_i^{k+T}} = 0$.
    \label{appn:admm:auglag_convergence}
\end{theorem}

\begin{proof}
\Cref{appn:admm:auglag_convergence} implies that the augmented Lagrangian decreases by a non-negative amount after every $T$ global iterations. Given the fact that every client will be updated at least once in the interval $[k, k + T]$, we conclude that the limit $\lim_{k \rightarrow \infty} \mathcal{L}(Z^{k+T}, \{ U_i^{k+T} \}, \{ Y_i^{k+T} \})$ exists and is at least $\underline{\gL}$.

Now we prove the second statement. From \Cref{eq:suff_dec} and the fact that $\widetilde{\gL}$ converges, we conclude that as $k \rightarrow \infty$, 
\begin{align*}
    \norm{Z^{k+T} - Z^{k}} \rightarrow 0, \quad \norm{U_i^{k+T} - U_i^{k}} \rightarrow 0.
\end{align*}
Combining this with \Cref{lemma:diff_dual}, we have $\norm{Y_i^{k+1} - Y_i^{k}} \rightarrow 0$. Based on the definition of $Y_i^{t+1}$, this implies that $$\norm{U_i^{k+1} - Z^{k+1}} \rightarrow 0$$ 
\end{proof}
\begin{remark}
\Cref{appn:admm:auglag_convergence} establishes that the sequence of primal and dual variables updated after each $T$ global iterations of \Cref{algo1} and \Cref{algo2} converges. Furthermore, we have $\norm{U_i^{k+1} - Z^{k+1}} \rightarrow 0$, i.e., the consensus constraint is satisfied.
\end{remark}

\subsection{Convergence to stationary point}
\label{ap:thrm_proof:auglag_stationary}

In the below theorem we present another guarantee that the limit of the sequence $(Z^{k}, \{ U_i^{k} \}, \{ Y_i^{k} \})$ is the a stationary solution for Problem \Cref{Prob:pca_decentralized_admm_nonlinear}.

\begin{theorem} 
    Suppose the assumptions in \Cref{appn:admm:auglag_convergence} hold. Then the limit point $(Z^{*}, \{ U_i^{*} \}, \{ Y_i^{*} \})$ of the sequence $(Z^{k}, \{ U_i^{k} \}, \{ Y_i^{k} \})$ is a stationary solution to Problem \Cref{Prob:pca_decentralized_admm_nonlinear}. That is, for all $i$,
    \begin{align*}
        \nabla f_i(Z^*) + Y_i^* &= 0, \\
        Z^* &= U_i^*.
    \end{align*}
    \label{appn:admm:auglag_convergence_stationary}
\end{theorem}
\begin{proof}
    See the proof to \cite[Theorem 2.4]{admm_nonconvex}. Here we make some remarks. First, because \textsc{FedPE} and \textsc{FedPG} allows for client sampling, the proof relies on an assumption that all clients will participate after some fixed number of rounds (in particular, $T$ rounds). Second, since local objectives are smooth (possible non-convex), the primal variables $U_i$ are updated using first-order methods like SGD or projected GD. Finally, the proof aims to show that after every $T$ rounds, we obtain a sufficient decrease in the augmented Lagrangian; coupled with the fact that the augmented Lagrangian is bounded below, the sequence of variables converges to a stationary point of $\gL$.
\end{proof}


==> other_packages.tex <==
%\usepackage[pdftex]{graphicx} % Required for including pictures
%\usepackage[pdftex,linkcolor=black,pdfborder={0 0 0}]{hyperref} % Format links for pdf
\usepackage{calc} % To reset the counter in the document after title page    
\usepackage{enumitem} % Includes lists

\usepackage{parskip}

% \usepackage[all]{nowidow} % Tries to remove widows
%\usepackage[protrusion=true,expansion=true]{microtype} % Improves typography, load after fontpackage is selected
\usepackage{algorithm}% http://ctan.org/pkg/algorithm
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx


\usepackage{times}
\usepackage{soul}
\usepackage{url}

\usepackage{setspace}
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
%\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage[detect-all]{siunitx}

\usepackage{xspace}
%\usepackage{caption}
\usepackage{subcaption}
\usepackage{bm}
\usepackage{array}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%Multi-line for Algorithm
\usepackage{algorithm,tabularx}
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}
\makeatletter
\newcommand{\multilines}[1]{%
	\begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
		#1
	\end{tabularx}
}
\makeatother

\usepackage{mathtools}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclareMathOperator{\myspan}{span}

\usepackage{amsthm}
\usepackage{multirow}
\usepackage{color}
\usepackage{epstopdf}
\usepackage{endnotes}
\usepackage{framed}
%\usepackage[keeplastbox]{flushend}
\usepackage{cool} % for partial derivative
\usepackage{enumerate} % for \begin{enumerate}[(a)], or [a)]
	%\usepackage{hyperref}
	%\usepackage{url}
	\usepackage[subnum]{cases}
	\usepackage{multicol}
	\usepackage{tablefootnote}
	
	% Special Defined Notation
	\DeclareMathOperator*{\argmax}{arg\,max}
	\DeclareMathOperator*{\argmin}{arg\,min}
	
	\newcommand{\note}[1]{\emph{\color{blue}#1}}
	\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.99mu#1\mkern-1.5mu}\mkern 1.5mu}
	
	\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}
	\DeclarePairedDelimiterX{\abs}[1]{\lvert}{\rvert}{#1}
	\DeclarePairedDelimiterX{\innProd}[1]{\langle}{\rangle}{#1}
	\DeclarePairedDelimiter\set{\lbrace}{\rbrace}
	
	\newcommand{\Prob}[1]{\ensuremath{\mathbb{P} \left[ #1 \right]}}
	\newcommand{\Ex}[1]{\ensuremath{\mathbb{E} \left[ #1 \right]}}
	\newcommand{\Avg}[2]{\ensuremath{\mathbb{E}_{#1} \left[ #2 \right]}}
	\newcommand{\La}[1]{\ensuremath{#1^{*}(s)}} %Laplace transform
	\newcommand{\PrimeN}[2][f]{\ensuremath{#1^{\prime #2}} \,}
	\newcommand{\SumNoLim}[2]{\ensuremath{\sum\nolimits_{#1}^{#2}}}
	\newcommand{\SumLim}[2]{\ensuremath{\sum\limits_{#1}^{#2}}}
	\newcommand{\Setm}[2]{\ensuremath{\{\,#1\mid#2\,\}} \,}
	\newcommand{\defeq}{\vcentcolon=}
	% similarly: \coloneqq
	\newcommand{\eqdef}{=\vcentcolon}
	% similarly: \eqqcolon
	\newcommand*\mean[1]{\bar{#1}}
	\newcommand{\mul}{\ensuremath{\,} \,}
	\newcommand{\pder}[2][]{\frac{\partial#1}{\partial#2}} % use: \pder[f]{x} and \pder{x} where f is optional
	
	\newcommand{\LeRiP}[1]{\ensuremath{\left(#1\right)}}
	\newcommand{\LeRiS}[1]{\ensuremath{\left[#1\right]}}
	\newcommand{\LeRiC}[1]{\ensuremath{\left\{#1\right\}}}
	\newcommand{\nbigP}[1]{\ensuremath{(#1)}}
	\newcommand{\nbigS}[1]{\ensuremath{[#1]}}
	\newcommand{\nbigC}[1]{\ensuremath{\{#1\}}}
	\newcommand{\bigP}[1]{\ensuremath{\bigl(#1\bigr)}}
	\newcommand{\bigS}[1]{\ensuremath{\bigl[#1\bigr]}}
	\newcommand{\bigC}[1]{\ensuremath{\bigl\{#1\bigr\}}}
	\newcommand{\biggP}[1]{\ensuremath{\biggl(#1\biggr)}}
	\newcommand{\biggS}[1]{\ensuremath{\biggl[#1\biggr]}}
	\newcommand{\biggC}[1]{\ensuremath{\biggl\{#1\biggr\}}}
	\newcommand{\BigP}[1]{\ensuremath{\Bigl(#1\Bigr)}}
	\newcommand{\BigS}[1]{\ensuremath{\Bigl[#1\Bigr]}}
	\newcommand{\BigC}[1]{\ensuremath{\Bigl\{#1\Bigr\}}}
	\newcommand{\BiggP}[1]{\ensuremath{\Biggl(#1\Biggr)}}
	\newcommand{\BiggS}[1]{\ensuremath{\Biggl[#1\Biggr]}}
	\newcommand{\BiggC}[1]{\ensuremath{\Biggl\{#1\Biggr\}}}
	% \bigm|, \Bigm|, \biggm|, and \Biggm|
	%%%%% Font commands
	\newcommand{\tbf}[1]{\textbf{#1}}% text bold
	\newcommand{\tit}{\textit}% text italic
	\newcommand{\tsl}{\textsl}% text slanted
	\newcommand{\tsc}{\textsc}% text small cap
	\newcommand{\ttt}{\texttt}% text typewriter
	\newcommand{\trm}{\textrm}% text roman
	\newcommand{\tsf}[1]{\textsf{#1}}% text sans serif
	\newcommand{\tup}{\textup}% text upright
	\newcommand{\mbf}{\mathbf}% math bold
	\providecommand{\mit}{\mathit}% math italic
	\newcommand{\msf}{\mathsf}% math sans serif
	\newcommand{\mrm}{\mathrm}% math roman
	\newcommand{\mtt}{\mathtt}% math typewriter
	\newcommand{\mybold}[1]{\ensuremath{\boldsymbol{#1}}}
	
	\newcommand{\centered}[1]{\begin{tabular}{l} #1 \end{tabular}} 
	
	\newcommand{\Bold}[1]{\boldsymbol{#1}} % Bold math symbol, use as \Bold{\alpha}
	\newcommand{\Cal}[1]{\mathcal{#1}} % phics - only caps, use as \Cal{A}
	\newcommand{\DD}[1]{\mathbb{#1}} % Doubled - blackboard bold - only caps, use as \DD{A}
	%\newcommand{\Euler}[1]{\mathscr{#1}} % Euler Script - only caps, use as \Euler{A}
	\newcommand{\Frak}[1]{\mathfrak{#1}} % Fraktur, use as \Frak{a}
	\newcommand{\blue}[1]{{\color{blue}#1}\xspace}
	\newcommand{\red}[1]{{\color{red}#1}\xspace}
	
	\theoremstyle{plain}
	\newtheorem{theorem}{Theorem}
	\newtheorem{assumption}{Assumption}
	\newtheorem{corollary}{Corollary}
	\newtheorem{lemma}{Lemma}
	\newtheorem{proposition}{Proposition}
	\theoremstyle{definition}
	\newtheorem{definition}{Definition}
	\newtheorem{remark}{Remark}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

==> packages.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{booktabs} % for professional tables
\usepackage{hyperref}


% Attempt to make hyperref and algorithmic work together better:
%\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:

% If accepted, instead use the following line for the camera-ready submission:

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{enumitem}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}
% if you use cleveref..
\usepackage{hyperref}
\usepackage{xr-hyper}


\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{assumption}[theorem]{Assumption}
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}

% Optional math commands from https://github.com/goodfeli/dlbook_notation.
\usepackage{hyperref}

\usepackage{url}
\usepackage{graphicx,wrapfig,lipsum} 
\usepackage{times}
\usepackage{soul}
\usepackage{url}
%\usepackage[utf8]{inputenc}
%\usepackage[small]{caption}
\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{booktabs}
\urlstyle{same}

\usepackage{mwe} % for blindtext and example-image-a in example
\usepackage{wrapfig}


\usepackage{setspace}
\usepackage{amsmath,amssymb,amsfonts}
\input{math_commands.tex}

\newcommand{\crefrangeconjunction}{--}
\crefformat{equation}{(#2#1#3)}
\crefrangeformat{equation}{(#3#1#4) to~(#5#2#6)}
\crefmultiformat{equation}{(#2#1#3)}%
{ and~(#2#1#3)}{, (#2#1#3)}{ and~(#2#1#3)}
\crefname{assumption}{assumption}{assumptions}
\crefname{Assumption}{Assumption}{Assumptions}
\usepackage{bbm}
\usepackage[mathscr]{euscript}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
% \usepackage[detect-all]{siunitx}

\usepackage{xspace}
\usepackage{caption}
\usepackage{subcaption}
\captionsetup{compatibility=false}
\usepackage{bm}
\usepackage{array}
\usepackage{multirow}

\makeatletter
\newcommand{\multilines}[1]{%
	\begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
		#1
	\end{tabularx}
}
\makeatother

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

\newcommand{\sigmahat}{\red{\hat{\sigma}}}
\newcommand{\OurAlg}{\ensuremath{\textsf{FeDEQ}}\xspace}
\Crefname{figure}{Fig.}{Figs.}
\Crefname{table}{Table}{Tables}
\Crefname{section}{Sec.}{Secs.}

\newcommand{\note}[1]{\emph{\color{blue}#1}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.99mu#1\mkern-1.5mu}\mkern 1.5mu}
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}
%\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\DeclarePairedDelimiterX{\abs}[1]{\lvert}{\rvert}{#1}
\newcommand{\innProd}[1]{\left\langle#1\right\rangle}
\newcommand{\set}[1]{\left\lbrace#1\right\rbrace}

\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
\DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
% \DeclarePairedDelimiterX{\innProd}[1]{\langle}{\rangle}{#1}
% \DeclarePairedDelimiter\set{\lbrace}{\rbrace}

\newcommand{\Prob}[1]{\ensuremath{\mathbb{P} \left[ #1 \right]}}
\newcommand{\Ex}[1]{\ensuremath{\mathbb{E} \left[ #1 \right]}}
\newcommand{\Avg}[2]{\ensuremath{\mathbb{E}_{#1} \left[ #2 \right]}}
\newcommand{\La}[1]{\ensuremath{#1^{*}(s)}} %Laplace transform
\newcommand{\PrimeN}[2][f]{\ensuremath{#1^{\prime #2}} \,}
\newcommand{\SumNoLim}[2]{\ensuremath{\sum\nolimits_{#1}^{#2}}}
\newcommand{\SumLim}[2]{\ensuremath{\sum\limits_{#1}^{#2}}}
\newcommand{\Setm}[2]{\ensuremath{\{\,#1\mid#2\,\}} \,}
\newcommand{\defeq}{\vcentcolon=}
% similarly: \coloneqq
\newcommand{\eqdef}{=\vcentcolon}
% similarly: \eqqcolon
\newcommand*\mean[1]{\bar{#1}}
\newcommand{\mul}{\ensuremath{\,} \,}
\newcommand{\pder}[2][]{\frac{\partial#1}{\partial#2}} % use: \pder[f]{x} and \pder{x} where f is optional

\newcommand{\LeRiP}[1]{\ensuremath{\left(#1\right)}}
\newcommand{\LeRiS}[1]{\ensuremath{\left[#1\right]}}
\newcommand{\LeRiC}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\nbigP}[1]{\ensuremath{(#1)}}
\newcommand{\nbigS}[1]{\ensuremath{[#1]}}
\newcommand{\nbigC}[1]{\ensuremath{\{#1\}}}
\newcommand{\bigP}[1]{\ensuremath{\bigl(#1\bigr)}}
\newcommand{\bigS}[1]{\ensuremath{\bigl[#1\bigr]}}
\newcommand{\bigC}[1]{\ensuremath{\bigl\{#1\bigr\}}}
\newcommand{\bigNorm}[1]{\ensuremath{\bigl\lVert#1\bigr\rVert}}
\newcommand{\biggP}[1]{\ensuremath{\biggl(#1\biggr)}}
\newcommand{\biggS}[1]{\ensuremath{\biggl[#1\biggr]}}
\newcommand{\biggC}[1]{\ensuremath{\biggl\{#1\biggr\}}}
\newcommand{\biggNorm}[1]{\ensuremath{\biggl\lVert#1\biggr\rVert}}
\newcommand{\BigP}[1]{\ensuremath{\Bigl(#1\Bigr)}}
\newcommand{\BigS}[1]{\ensuremath{\Bigl[#1\Bigr]}}
\newcommand{\BigC}[1]{\ensuremath{\Bigl\{#1\Bigr\}}}
\newcommand{\BigNorm}[1]{\ensuremath{\Bigl\lVert#1\Bigr\rVert}}
\newcommand{\BiggP}[1]{\ensuremath{\Biggl(#1\Biggr)}}
\newcommand{\BiggS}[1]{\ensuremath{\Biggl[#1\Biggr]}}
\newcommand{\BiggC}[1]{\ensuremath{\Biggl\{#1\Biggr\}}}
\newcommand{\BiggNorm}[1]{\ensuremath{\Biggl\lVert#1\Biggr\rVert}}
% \bigm|, \Bigm|, \biggm|, and \Biggm|
%%%%% Font commands
\DeclareUnicodeCharacter{FB01}{fi}
\newcommand{\tbf}[1]{\textbf{#1}}% text bold
\newcommand{\tit}{\textit}% text italic
\newcommand{\tsl}{\textsl}% text slanted
\newcommand{\tsc}{\textsc}% text small cap
\newcommand{\ttt}{\texttt}% text typewriter
\newcommand{\trm}{\textrm}% text roman
\newcommand{\tsf}[1]{\textsf{#1}}% text sans serif
\newcommand{\tup}{\textup}% text upright
\newcommand{\mbf}{\mathbf}% math bold
\providecommand{\mit}{\mathit}% math italic
\newcommand{\msf}{\mathsf}% math sans serif
\newcommand{\mrm}{\mathrm}% math roman
\newcommand{\mtt}{\mathtt}% math typewriter
\newcommand{\mybold}[1]{\ensuremath{\boldsymbol{#1}}}
\DeclareMathOperator{\Ima}{Im}

\newcommand{\centered}[1]{\begin{tabular}{l} #1 \end{tabular}}

\newcommand{\Bold}[1]{\boldsymbol{#1}} % Bold math symbol, use as \Bold{\alpha}
\newcommand{\Cal}[1]{\mathcal{#1}} % phics - only caps, use as \Cal{A}
\newcommand{\DD}[1]{\mathbb{#1}} % Doubled - blackboard bold - only caps, use as \DD{A}
%\newcommand{\Euler}[1]{\mathscr{#1}} % Euler Script - only caps, use as \Euler{A}
\newcommand{\Frak}[1]{\mathfrak{#1}} % Fraktur, use as \Frak{a}
\newcommand{\blue}[1]{{\color{blue}#1}\xspace}
\newcommand{\red}[1]{{\color{red}#1}\xspace}
\newcommand{\josh}[1]{{\color{red}#1}\xspace}
\newcommand{\verify}[1]{{\color{red}#1}\xspace}
%Personal
%\newcommand{\ellZf}[1]{\ensuremath{\ell(z_i; \theta)}}

\newcommand{\up}{\texttt{up}\xspace}
\newcommand{\mt}{\texttt{mt}\xspace}
\newcommand{\sv}{\texttt{sv}\xspace}


\newcommand{\LineComment}[1]{\quad \texttt{// #1}}
